Measurement of charge-dependent directed flow in STAR Beam Energy Scan (BES-II) Au+Au and U+U collisions

We presented the rapidity dependence of directed flow ($v_1$) and its slope ($dv_1/dy$) for $\pi^\pm$, $K^\pm$ and $p(\bar{p}$) in Au+Au collisions at $\sqrt{s_{NN}}$ = 7.7 -- 19.6 GeV from the Beam Energy Scan Phase-II, as well as in U+U collisions at $\sqrt{s_{NN}}$ = 193 GeV measured by the STAR experiment. The $v_1$ values are reported as a function of rapidity and centrality. Additionally, the $dv_1/dy$ and the charge dependent difference, $\Delta(dv_1/dy)$, of the three identified particles in U+U collisions is compared to those in Au+Au and isobar (Ru+Ru and Zr+Zr) collisions. These findings offer insights into the initial electromagnetic field as well as baryon transport at various system sizes and beam energies.

==> bib.tex <==
@article{1,
  title = {Charge-dependent flow induced by magnetic and electric fields in heavy ion collisions},
  author = {G\"ursoy, Umut and Kharzeev, Dmitri and Marcus, Eric and Rajagopal, Krishna and Shen, Chun},
  journal = {Phys. Rev. C},
  volume = {98},
  issue = {5},
  pages = {055201},
  numpages = {15},
  year = {2018},
  month = {Nov},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevC.98.055201},
  url = {https://link.aps.org/doi/10.1103/PhysRevC.98.055201}
}
@article{2,
  title = {Magnetohydrodynamics, charged currents, and directed flow in heavy ion collisions},
  author = {G\"ursoy, Umut and Kharzeev, Dmitri and Rajagopal, Krishna},
  journal = {Phys. Rev. C},
  volume = {89},
  issue = {5},
  pages = {054905},
  numpages = {12},
  year = {2014},
  month = {May},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevC.89.054905},
  url = {https://link.aps.org/doi/10.1103/PhysRevC.89.054905}
}
@article{3,
  title = {Elliptical Flow: A Signature for Early Pressure in Ultrarelativistic Nucleus-Nucleus Collisions},
  author = {Sorge, Heinz},
  journal = {Phys. Rev. Lett.},
  volume = {78},
  issue = {12},
  pages = {2309--2312},
  numpages = {0},
  year = {1997},
  month = {Mar},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevLett.78.2309},
  url = {https://link.aps.org/doi/10.1103/PhysRevLett.78.2309}
}
@article{4,
  title = {Observation of the Electromagnetic Field Effect via Charge-Dependent Directed Flow in Heavy-Ion Collisions at the Relativistic Heavy Ion Collider},
  author = {Abdulhamid, M. I. and Aboona, B. E. and Adam, J. and Adams, J. R. and Agakishiev, G. and Aggarwal, I. and Aggarwal, M. M. and Ahammed, Z. and Aitbaev, A. and Alekseev, I. and Alpatov, E. and Aparin, A. and Aslam, S. and Atchison, J. and Averichev, G. S. and Bairathi, V. and Ball Cap, J. G. and Barish, K. and Bhagat, P. and Bhasin, A. and Bhatta, S. and Bhosale, S. R. and Bordyuzhin, I. G. and Brandenburg, J. D. and Brandin, A. V. and Cai, X. Z. and Caines, H. and Calder\'on de la Barca S\'anchez, M. and Cebra, D. and Ceska, J. and Chakaberia, I. and Chan, B. K. and Chang, Z. and Chatterjee, A. and Chen, D. and Chen, J. and Chen, J. H. and Chen, Z. and Cheng, J. and Cheng, Y. and Choudhury, S. and Christie, W. and Chu, X. and Crawford, H. J. and Dale-Gau, G. and Das, A. and Dash, A. P. and Daugherity, M. and Dedovich, T. G. and Deppner, I. M. and Derevschikov, A. A. and Dhamija, A. and Dixit, P. and Dong, X. and Drachenberg, J. L. and Duckworth, E. and Dunlop, J. C. and Engelage, J. and Eppley, G. and Esumi, S. and Evdokimov, O. and Eyser, O. and Fatemi, R. and Fazio, S. and Feng, C. J. and Feng, Y. and Finch, E. and Fisyak, Y. and Flor, F. A. and Fu, C. and Gao, T. and Geurts, F. and Ghimire, N. and Gibson, A. and Gopal, K. and Gou, X. and Grosnick, D. and Gupta, A. and Hamed, A. and Han, Y. and Harasty, M. D. and Harris, J. W. and Harrison-Smith, H. and He, W. and He, X. H. and He, Y. and Hu, C. and Hu, Q. and Hu, Y. and Huang, H. and Huang, H. Z. and Huang, S. L. and Huang, T. and Huang, X. and Huang, Y. and Huang, Y. and Humanic, T. J. and Isenhower, D. and Isshiki, M. and Jacobs, W. W. and Jalotra, A. and Jena, C. and Ji, Y. and Jia, J. and Jin, C. and Ju, X. and Judd, E. G. and Kabana, S. and Kalinkin, D. and Kang, K. and Kapukchyan, D. and Kauder, K. and Keane, D. and Kechechyan, A. and Kiselev, A. and Knospe, A. G. and Ko, H. S. and Kochenda, L. and Korobitsin, A. A. and Kraeva, A. Yu. and Kravtsov, P. and Kumar, L. and Labonte, M. C. and Lacey, R. and Landgraf, J. M. and Lebedev, A. and Lednicky, R. and Lee, J. H. and Leung, Y. H. and Lewis, N. and Li, C. and Li, H-S. and Li, W. and Li, X. and Li, Y. and Li, Y. and Li, Z. and Liang, X. and Liang, Y. and Lin, T. and Lin, Y. and Liu, C. and Liu, F. and Liu, G. and Liu, H. and Liu, L. and Liu, T. and Liu, X. and Liu, Y. and Liu, Z. and Ljubicic, T. and Lomicky, O. and Longacre, R. S. and Loyd, E. M. and Lu, T. and Lukow, N. S. and Luo, X. F. and Luong, V. B. and Ma, L. and Ma, R. and Ma, Y. G. and Magdy, N. and Mallick, D. and Margetis, S. and Matis, H. S. and McNamara, G. and Mi, K. and Minaev, N. G. and Mohanty, B. and Mondal, M. M. and Mooney, I. and Morozov, D. A. and Mudrokh, A. and Nagy, M. I. and Nain, A. S. and Nam, J. D. and Nasim, M. and Nedorezov, E. and Neff, D. and Nelson, J. M. and Nemes, D. B. and Nie, M. and Nigmatkulov, G. and Niida, T. and Nogach, L. V. and Nonaka, T. and Odyniec, G. and Ogawa, A. and Oh, S. and Okorokov, V. A. and Okubo, K. and Page, B. S. and Pak, R. and Pandav, A. and Panebratsev, Y. and Pani, T. and Parfenov, P. and Paul, A. and Perkins, C. and Pokhrel, B. R. and Posik, M. and Povarov, A. and Protzman, T. and Pruthi, N. K. and Putschke, J. and Qin, Z. and Qiu, H. and Quintero, A. and Racz, C. and Radhakrishnan, S. K. and Rana, A. and Ray, R. L. and Ritter, H. G. and Robertson, C. W. and Rogachevsky, O. V. and Rosales Aguilar, M. A. and Roy, D. and Ruan, L. and Sahoo, A. K. and Sahoo, N. R. and Sako, H. and Salur, S. and Samigullin, E. and Sato, S. and Schaefer, B. C. and Schmidke, W. B. and Schmitz, N. and Seger, J. and Seto, R. and Seyboth, P. and Shah, N. and Shahaliev, E. and Shanmuganathan, P. V. and Shao, T. and Sharma, M. and Sharma, N. and Sharma, R. and Sharma, S. R. and Sheikh, A. I. and Shen, D. and Shen, D. Y. and Shen, K. and Shi, S. S. and Shi, Y. and Shou, Q. Y. and Si, F. and Singh, J. and Singha, S. and Sinha, P. and Skoby, M. J. and S\"ohngen, Y. and Song, Y. and Srivastava, B. and Stanislaus, T. D. S. and Stewart, D. J. and Strikhanov, M. and Stringfellow, B. and Su, Y. and Sun, C. and Sun, X. and Sun, Y. and Sun, Y. and Surrow, B. and Svirida, D. N. and Sweger, Z. W. and Tamis, A. C. and Tang, A. H. and Tang, Z. and Taranenko, A. and Tarnowsky, T. and Thomas, J. H. and Tlusty, D. and Todoroki, T. and Tokarev, M. V. and Trentalange, S. and Tribedy, P. and Tripathy, S. K. and Tsai, O. D. and Tsang, C. Y. and Tu, Z. and Tyler, J. and Ullrich, T. and Underwood, D. G. and Upsal, I. and Van Buren, G. and Vasiliev, A. N. and Verkest, V. and Videb\ae{}k, F. and Vokal, S. and Voloshin, S. A. and Wang, F. and Wang, G. and Wang, J. S. and Wang, J. and Wang, X. and Wang, Y. and Wang, Y. and Wang, Y. and Wang, Z. and Webb, J. C. and Weidenkaff, P. C. and Westfall, G. D. and Wieman, H. and Wilks, G. and Wissink, S. W. and Wu, J. and Wu, J. and Wu, X. and Wu, X. and Xi, B. and Xiao, Z. G. and Xie, G. and Xie, W. and Xu, H. and Xu, N. and Xu, Q. H. and Xu, Y. and Xu, Y. and Xu, Z. and Xu, Z. and Yan, G. and Yan, Z. and Yang, C. and Yang, Q. and Yang, S. and Yang, Y. and Ye, Z. and Ye, Z. and Yi, L. and Yip, K. and Yu, Y. and Zha, W. and Zhang, C. and Zhang, D. and Zhang, J. and Zhang, S. and Zhang, W. and Zhang, X. and Zhang, Y. and Zhang, Y. and Zhang, Y. and Zhang, Y. and Zhang, Z. J. and Zhang, Z. and Zhang, Z. and Zhao, F. and Zhao, J. and Zhao, M. and Zhou, C. and Zhou, J. and Zhou, S. and Zhou, Y. and Zhu, X. and Zurek, M. and Zyzak, M.},
  collaboration = {STAR Collaboration},
  journal = {Phys. Rev. X},
  volume = {14},
  issue = {1},
  pages = {011028},
  numpages = {12},
  year = {2024},
  month = {Feb},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevX.14.011028},
  url = {https://link.aps.org/doi/10.1103/PhysRevX.14.011028}
}
@article{5,
  title = {Directed flow of transported and nontransported protons in Au $+$ Au collisions from an ultrarelativistic quantum molecular dynamics model},
  author = {Guo, Yao and Liu, Feng and Tang, Aihong},
  journal = {Phys. Rev. C},
  volume = {86},
  issue = {4},
  pages = {044901},
  numpages = {4},
  year = {2012},
  month = {Oct},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevC.86.044901},
  url = {https://link.aps.org/doi/10.1103/PhysRevC.86.044901}
}
@article{6,
  title = {Energy dependence study of directed flow in $\mathrm{Au}+\mathrm{Au}$ collisions using an improved coalescence in a multiphase transport model},
  author = {Nayak, Kishora and Shi, Shusu and Xu, Nu and Lin, Zi-Wei},
  journal = {Phys. Rev. C},
  volume = {100},
  issue = {5},
  pages = {054903},
  numpages = {8},
  year = {2019},
  month = {Nov},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevC.100.054903},
  url = {https://link.aps.org/doi/10.1103/PhysRevC.100.054903}
}
@article{7,
  title = {Splitting of proton-antiproton directed flow in relativistic heavy-ion collisions},
  author = {Bo\ifmmode \dot{z}\else \.{z}\fi{}ek, Piotr},
  journal = {Phys. Rev. C},
  volume = {106},
  issue = {6},
  pages = {L061901},
  numpages = {5},
  year = {2022},
  month = {Dec},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevC.106.L061901},
  url = {https://link.aps.org/doi/10.1103/PhysRevC.106.L061901}
}
@article{8,
	author = {{Prasad Dash, Aditya}},
	title = {Exploring electromagnetic field effects and constraining transport parameters of QGP using STAR BES-II data},
	DOI= "10.1051/epjconf/202429610007",
	url= "https://doi.org/10.1051/epjconf/202429610007",
	journal = {EPJ Web Conf.},
	year = 2024,
	volume = 296,
	pages = "10007",
}
@misc{9,
      title={Electric charge and strangeness-dependent directed flow splitting of produced quarks in Au+Au collisions}, 
      author={STAR Collaboration},
      year={2023},
      eprint={2304.02831},
      archivePrefix={arXiv},
      primaryClass={nucl-ex},
      url={https://arxiv.org/abs/2304.02831}, 
}
@misc{10,
      title={Baryon inhomogeneities driven charge dependent directed flow in heavy ion collisions}, 
      author={Tribhuban Parida and Sandeep Chatterjee},
      year={2023},
      eprint={2305.08806},
      archivePrefix={arXiv},
      primaryClass={nucl-th},
      url={https://arxiv.org/abs/2305.08806}, 
}
